An open-source finite element toolbox for anisotropic creep and irradiation growth: Application to tube and spacer grid assembly

This work presents an open-source interface that couples the viscoplastic self-consistent (VPSC) model capable of simulating anisotropic creep and irradiation growth in polycrystalline materials with the finite element solver Code_Aster. The interface enables the simulation of the micromechanical response of irradiated zirconium alloy components by integrating grain-level constitutive behavior into a structural FEM framework. A key feature is the automated rotation of stress and strain tensors between the global FEM frame and the local crystallographic axes, a transformation not natively supported by Code_Aster. The elastic strain is recovered analytically using the inverse of the self-consistently stiffness tensor provided by VPSC. As a demonstration, the framework is applied to an actual model of a pressurized water reactor (PWR) spacer grid, based on a patented design, capturing nonlinear contact and the anisotropic response of the cladding and grid. Simulations reveal the micromechanisms controlling the evolution of clearance between components and highlight the role of crystallographic texture in mitigating wear. In particular, a texture with a high fraction of prismatic planes oriented in the normal direction of the grid appears to be the most suitable for spacer design, as it minimizes clearance and contributes to wear resistance. The interface offers a flexible, extensible platform for high-fidelity simulations in nuclear fuel performance analysis.

==> Intro_merge.tex <==
A precise and reliable simulation of nuclear fuel behavior requires an accurate description of the cladding’s mechanical response under irradiation and complex mechanical loads. Conventional fuel performance codes typically rely on empirical constitutive models calibrated for specific materials and service conditions, which limits their predictive capabilities when applied to modern cladding designs or scenarios involving increased mechanical demands. At the same time, the availability of open-source, validated simulation platforms has become a decisive factor for advancing nuclear engineering in a transparent and reproducible manner.

In nuclear fuel rod assemblies, the fuel elements (uranium pellets encapsulated in cladding tubes) are held in place by a spacer grid. In some pressurized water reactors (PWRs), this structure features a hexagonal housing in its central region that accommodates the fuel rod, characterized by its geometric symmetry and the arrangement of spring and dimple sheets that ensure mechanical contact with the cladding (see Fig. \ref{fig:FlexibleSpacerGrid}). 
Under reactor operating conditions, the fuel rod assembly experiences significant irradiation doses. In zirconium alloy components (cladding tube and grid), these conditions induce dimensional changes through creep and irradiation growth~\cite{fidleris1988irradiation}. Consequently, irradiation-driven deformation may lead to loss of contact between the cladding tube and the spacer grid’s springs/dimples. This phenomenon, in combination with the vibrations produced by the coolant, contributes to the deterioration of the component's integrity. This phenomenon leads to the deterioration of the cladding tube surface.~\cite{kim2009impact, yan2011new, kim2008geometry, choi2004vibration}. Fretting wear between the grid and the cladding is a key concern in the design and operation of fuel rod assemblies in nuclear reactors~\cite{kim2010study}.

\begin{figure}[h!] 
	\centering
	\includegraphics[width=0.24\textwidth]{fig1.png}
	\caption{Flexible Spacer Grid  \citep{CONUAR}.}  
	\label{fig:FlexibleSpacerGrid}
\end{figure}

In most of the studies mentioned above, models were developed in which creep and irradiation-induced growth were treated independently, without coupling the interactions between both phenomena. That is, a predefined separation is assumed to account for the gap induced by irradiation, but the underlying mechanisms contributing to this behavior remain poorly understood. Subsequent efforts moved toward coupled models that simultaneously integrate creep and irradiation growth and aim to predict the separation between the cladding and the grid. However, some ot these models are still based on phenomenological approaches (see~\cite{billerey2005evolution}), which limits their applicability to narrow operating ranges and prevents them from properly capturing the influence of microstructure and material history—such as prior mechanical working or manufacturing processes.

Creep and irradiation-induced growth are material- and microstructure-dependent phenomena, and have been extensively studied~\citep{fidleris1988irradiation, griffiths1995microstructural}. A more recent contribution by \cite{patra2017crystal} presents a crystal plasticity constitutive framework to model these phenomena in polycrystals with a hexagonal close-packed (HCP) crystal structure, specifically zirconium and its alloys. The numeric model has been demonstrated to successfully capture the generation of point defects during irradiation, as well as the interaction that occurs between these defects with linear dislocations and grain boundaries. Furthermore, it has been demonstrated to effectively capture the process of dislocation loop nucleation and subsequent growth. The aforementioned phenomena contribute to the deformation of the single crystal, herein referred to as \textit{grain}. The open source VPSC $-ViscoPlastic Self Consistent-$ provides the grain interaction and the resulting polycrystal response~\cite{tome2023material}. VPSC considers crystalline texture and its effects, as well as microstructure evolution due to growth and creep under irradiation. A proprietary licensed finite element (FEM) solver is used to solve the problem at the macro level.

In this context, this work presents an open-source toolbox that integrates the micromechanics models in VPSC describing the physics of creep and irradiation-induced growth into the open-source FEM solver Code\_Aster (CAFEM) \citep{ASTER}, enabling the resolution of texture-dependent deformation in each component. This implementation extends the capabilities of a robust Finite Element platform, with over three decades of collaborative development and comprehensive verification, to code complex material phenomena in a modular open-source environment. The current version of the interface integrates the models on ~\cite{tome2023material} to simulate the anisotropic mechanical behavior by accounting for crystallographic texture and dislocation mechanisms, offering a more physically grounded alternative to semi-empirical approaches already present in Code_Aster. The coupling approach assumes an additive decomposition of the strain increment, accounting for both viscoplastic behavior from VPSC and elastic behavior from the FEM analysis ~\citep{llubel2024integracion},.


Code_Aster, in its standard configuration, does not perform the necessary tensor rotations or mappings between the global frame and the local crystallographic axes. The developed interface addresses this limitation by automating the transformation of stress and strain tensors between both frames at each integration point, enabling scalable simulations involving millions of Gauss points. Its validity is demonstrated through comparisons with benchmark results from \cite{patra2017crystal} for irradiated Zircaloy cladding, and extended to a full-scale industrial geometry: the spacer grid of a pressurized water reactor (PWR) fuel assembly, modeled with its current patented design. This showcases the capability of the proposed framework to capture nonlinear contact between the cladding tube and the spacer grid, as well as anisotropic material behavior, all within a fully open-source environment.

% A complementary function of this interface is the rotation of stress and strain tensors to a common coordinate system so they can be properly handled by the FEM solver. This implementation is used to investigate the interactions between the dimples of the spacer grid and the cladding tube, assuming a nonlinear kinematic contact condition between both components. This type of contact allows for a more realistic capture of the progressive evolution of clearance, in combination with the polycrystalline model that couples both creep and irradiation-induced growth. The predicted separation from these simulations can be used to assess the resulting wear behavior and to guide the design of nuclear fuel rod assemblies.

The modular architecture of the interface allows for future extensions, including deformation due to thermal expansion, thermal creep, rate-dependent plasticity, and precipitation hardening, as well as an extension of the elastic regime within VPSC, which remains limited in its standalone open-access version. This work thus contributes a flexible and reproducible toolset for high-fidelity structural analyses in nuclear engineering.


